Measuring the magnetic field of young stars using iSHELL observations: BP Tau and V347 Aur

While it has been suggested that there is a connection between the magnetic properties and the internal structure of young stars, there have not been enough magnetic measurements to firmly establish such a correlation at the earliest ages. Here, we contribute to this endeavor by presenting stellar parameters and magnetic field strength measurements of BP Tau and V347 Aur, both stars observed with the near-infrared spectrograph iSHELL. We first test the accuracy of our method by fitting synthetic stellar spectra to a sample of nine main and post-main-sequence stars. We report uncertainties of $\sigma_{\rm Teff}$ = 91 K in temperature and $\sigma_{\rm log(g)}$ = 0.14 in gravity. We then apply the modeling technique to BP Tau and measure a surface magnetic field strength of $\langle \rm B \rangle $ = 2.5$^{+0.15}_{-0.16}$ kG, confirming literature results. For this star, however, we obtain a much lower temperature value than previous optical studies ($\Delta \rm T \sim 400$ K) and interpret this significant temperature difference as due to the relatively higher impact of starspots at near-infrared wavelengths than at optical wavelengths. We further apply this technique to the class I protostellar source V347 Aur and measure for the first time its magnetic field strength $\langle \rm B \rangle = $ 1.36$^{+0.06}_{-0.05}$ kG and its surface gravity log(g) = 3.25$^{+0.14}_{-0.14}$. Lastly, we combine our measurements with pre-main-sequence stellar evolutionary models and illustrate the effects produced by starspots on the retrieved masses and ages of young stars.

==> Derived_stellar_mass_and_age.tex <==


\begin{table*}[!hbt]
   \centering
   \caption{Mass and age derivation using evolutionary models} \label{tab:evolutionary_models}
   \begin{tabular}{c | c c | c c}
      \toprule
       & \multicolumn{2}{c}{BP Tau} & \multicolumn{2}{c}{V347 Aur} \\
      \midrule
      Evolutionary Model & Magnetic & Non-magnetic & Magnetic & Non-magnetic \\
       \hline
      Age (Myr) & $11^{+11}_{-6}$ & $9^{+6}_{-4}$ & $1.0^{+0.8}_{?}$ & $1.0^{+0.6}_{?}$ \\
      Mass (M$_{\odot}$) & $0.82^{+0.14}_{-0.12}$ & $0.6^{+0.1}_{-0.08}$ & $0.42^{?}_{-0.12}$ & $0.25^{+0.04}_{-0.06}$ \\
      \bottomrule
   \end{tabular}
\end{table*}


==> Magnetic-field-detection-limit.tex <==

\begin{table*}[!hbt]
   \centering
   \caption{Comparison between the magnetic models and the non-magnetic models (\overrightarrow{\rm B} = 0 kG) for the Sun.} \label{tab:magnetic-detection-limits}
   \begin{tabular}{l | c c c}
      \toprule
     Stellar  & \multicolumn{3}{c}{Sun} \\
      %\midrule
     parameters  & Non-magnetic Model & Magnetic Model & Actual Values \\
       \hline
      T$_{\rm eff}$ (K) & 5807$^{+60}_{-154}$ & 5865$^{+93}_{-128}$ & 5778 \\
      log(g) & 4.44$^{+0.03}_{-0.02}$ & 4.43$^{+0.03}_{-0.02}$ & 4.43  \\
      $\langle \rm \overrightarrow{\rm B} \rangle$ (kG) & - & 0.12$^{+0.06}_{-0.07}$ & 0.001  \\
      $\rm [M/H]$ & 0.04$^{+0.02}_{-0.02}$ & 0.03$^{+0.02}_{-0.02}$ &0.0 \\
      $v\sin(i)$ (km s$^{-1}$) & $<$4 & $<$4 & 2.06\tablenotemark{a} \\
      $v_{turb}$ (km s$^{-1}$)  & 1.00$^{+0.07}_{-0.08}$  & 0.83$^{+0.09}_{-0.11}$ & 1.0  \\
      \bottomrule
   \end{tabular}
   \tablenotetext{a}{Rotational velocity measured at the solar equator.}
\end{table*}
